Efficient Calculation of the Joint Distribution of Order Statistics

We consider the problem of computing the joint distribution of order statistics of stochastically independent random variables in one- and two-group models. While recursive formulas for evaluating the joint cumulative distribution function of such order statistics exist in the literature for a longer time, their numerical implementation remains a challenging task. We tackle this task by presenting novel generalizations of known recursions which we utilize to obtain exact results (calculated in rational arithmetic) as well as faithfully rounded results. Finally, some applications in stepwise multiple hypothesis testing are discussed.

==> average_power.tex <==
% latex table generated in R 3.4.2 by xtable 1.8-3 package
% Fri Nov 16 11:09:17 2018
\begin{table}[ht]
\centering
\begin{tabular}{lrrrrrr}
  \hline
 & 0 & 1 & 2 & 3 & 4 & 5 \\ 
  \hline
2 & 0.56539 & 0.50342 &  &  &  &  \\ 
  3 & 0.54576 & 0.49842 & 0.44439 &  &  &  \\ 
  4 & 0.53446 & 0.49583 & 0.45256 & 0.40451 &  &  \\ 
  5 & 0.52712 & 0.49440 & 0.45819 & 0.41837 & 0.37494 &  \\ 
  6 & 0.52201 & 0.49357 & 0.46241 & 0.42840 & 0.39148 & 0.35175 \\ 
  7 & 0.51827 & 0.49310 & 0.46574 & 0.43606 & 0.40399 & 0.36955 \\ 
  8 & 0.51543 & 0.49285 & 0.46846 & 0.44214 & 0.41383 & 0.38349 \\ 
  9 & 0.51320 & 0.49273 & 0.47073 & 0.44710 & 0.42178 & 0.39473 \\ 
  10 & 0.51142 & 0.49270 & 0.47266 & 0.45124 & 0.42836 & 0.40398 \\ 
  11 & 0.50997 & 0.49272 & 0.47434 & 0.45475 & 0.43390 & 0.41174 \\ 
  12 & 0.50877 & 0.49278 & 0.47580 & 0.45777 & 0.43863 & 0.41833 \\ 
  13 & 0.50776 & 0.49286 & 0.47709 & 0.46039 & 0.44271 & 0.42401 \\ 
  14 & 0.50690 & 0.49295 & 0.47823 & 0.46268 & 0.44627 & 0.42895 \\ 
  15 & 0.50616 & 0.49306 & 0.47925 & 0.46472 & 0.44941 & 0.43329 \\ 
  16 & 0.50552 & 0.49316 & 0.48018 & 0.46653 & 0.45219 & 0.43712 \\ 
  17 & 0.50497 & 0.49327 & 0.48101 & 0.46815 & 0.45467 & 0.44053 \\ 
  18 & 0.50447 & 0.49338 & 0.48177 & 0.46962 & 0.45690 & 0.44358 \\ 
  19 & 0.50404 & 0.49348 & 0.48246 & 0.47094 & 0.45891 & 0.44634 \\ 
  20 & 0.50365 & 0.49358 & 0.48309 & 0.47215 & 0.46074 & 0.44883 \\ 
  21 & 0.50330 & 0.49368 & 0.48367 & 0.47325 & 0.46240 & 0.45109 \\ 
  22 & 0.50298 & 0.49378 & 0.48421 & 0.47427 & 0.46392 & 0.45316 \\ 
  23 & 0.50269 & 0.49387 & 0.48471 & 0.47520 & 0.46532 & 0.45505 \\ 
  24 & 0.50243 & 0.49395 & 0.48517 & 0.47605 & 0.46660 & 0.45679 \\ 
  25 & 0.50219 & 0.49404 & 0.48559 & 0.47685 & 0.46779 & 0.45840 \\ 
  26 & 0.50198 & 0.49412 & 0.48599 & 0.47759 & 0.46889 & 0.45988 \\ 
  27 & 0.50178 & 0.49420 & 0.48637 & 0.47828 & 0.46991 & 0.46126 \\ 
  28 & 0.50159 & 0.49427 & 0.48671 & 0.47892 & 0.47086 & 0.46254 \\ 
  29 & 0.50142 & 0.49434 & 0.48704 & 0.47952 & 0.47175 & 0.46373 \\ 
  30 & 0.50126 & 0.49441 & 0.48735 & 0.48008 & 0.47258 & 0.46485 \\ 
  31 & 0.50111 & 0.49447 & 0.48764 & 0.48060 & 0.47336 & 0.46589 \\ 
  32 & 0.50097 & 0.49453 & 0.48791 & 0.48110 & 0.47409 & 0.46687 \\ 
  33 & 0.50084 & 0.49459 & 0.48817 & 0.48157 & 0.47478 & 0.46779 \\ 
  34 & 0.50072 & 0.49465 & 0.48841 & 0.48201 & 0.47542 & 0.46866 \\ 
  35 & 0.50060 & 0.49470 & 0.48864 & 0.48242 & 0.47604 & 0.46948 \\ 
  36 & 0.50050 & 0.49475 & 0.48886 & 0.48282 & 0.47661 & 0.47025 \\ 
  37 & 0.50040 & 0.49480 & 0.48907 & 0.48319 & 0.47716 & 0.47098 \\ 
  38 & 0.50030 & 0.49485 & 0.48926 & 0.48354 & 0.47768 & 0.47167 \\ 
  39 & 0.50021 & 0.49489 & 0.48945 & 0.48388 & 0.47817 & 0.47233 \\ 
  40 & 0.50012 & 0.49494 & 0.48963 & 0.48420 & 0.47864 & 0.47295 \\ 
  41 & 0.50004 & 0.49498 & 0.48980 & 0.48451 & 0.47909 & 0.47354 \\ 
  42 & 0.49996 & 0.49502 & 0.48996 & 0.48480 & 0.47951 & 0.47411 \\ 
  43 & 0.49989 & 0.49506 & 0.49012 & 0.48508 & 0.47992 & 0.47465 \\ 
  44 & 0.49982 & 0.49509 & 0.49027 & 0.48534 & 0.48031 & 0.47516 \\ 
  45 & 0.49975 & 0.49513 & 0.49041 & 0.48559 & 0.48068 & 0.47565 \\ 
  46 & 0.49969 & 0.49516 & 0.49055 & 0.48584 & 0.48103 & 0.47612 \\ 
  47 & 0.49963 & 0.49520 & 0.49068 & 0.48607 & 0.48137 & 0.47657 \\ 
  48 & 0.49957 & 0.49523 & 0.49081 & 0.48629 & 0.48169 & 0.47700 \\ 
  49 & 0.49951 & 0.49526 & 0.49093 & 0.48651 & 0.48201 & 0.47741 \\ 
  50 & 0.49946 & 0.49529 & 0.49104 & 0.48672 & 0.48230 & 0.47781 \\ 
   \hline
\end{tabular}
\end{table}

